A path forward: Improving Internet routing security by enabling zones of trust

Although Internet routing security best practices have recently seen auspicious increases in uptake, ISPs have limited incentives to deploy them. They are operationally complex and expensive to implement, provide little competitive advantage, and protect only against origin hijacks, leaving unresolved the more general threat of path hijacks. We propose a new approach that achieves four design goals: improved incentive alignment to implement best practices; protection against path hijacks; expanded scope of such protection to customers of those engaged in the practices; and reliance on existing capabilities rather than needing complex new software in every participating router. Our proposal leverages an existing coherent core of interconnected ISPs to create a zone of trust, a topological region that protects not only all networks in the region, but all directly attached customers of those networks. Customers benefit from choosing ISPs committed to the practices, and ISPs thus benefit from committing to the practices. We compare our approach to other schemes, and discuss how a related proposal, ASPA, could be used to increase the scope of protection our scheme achieves. We hope this proposal inspires discussion of how the industry can make practical, measurable progress against the threat of route hijacks in the short term by leveraging institutionalized cooperation rooted in transparency and accountability.

==> Makefile <==
TEX=			vipzone.tex abstract.tex introduction.tex \
			background.tex threat.tex design-principles.tex \
			solution.tex discussion.tex comparison.tex \
			conclusion.tex appendix-hurricane.tex deployment.tex

FIGURES=		figures/vipzone-0.pdf \
			figures/vipzone-1.pdf \
			figures/vipzone-2.pdf \
			figures/vipzone-3.pdf \
			figures/vipzone-4.pdf \
			figures/vipzone-5.pdf \
			figures/vipzone-6.pdf \
			figures/vipzone-7.pdf \
			figures/vipzone-size-defn.pdf

vipzone.pdf:		${TEX} ${FIGURES} bib.bib
			pdflatex vipzone
			bibtex vipzone
			pdflatex vipzone
			pdflatex vipzone
			pdflatex vipzone

clean:
			rm -f vipzone.pdf vipzone.aux vipzone.blg vipzone.log \
				vipzone.bbl vipzone.out vipzone.toc *~ *.bak


==> deployment.tex <==
\section{Deployment Trajectories}
\label{sec:deployment}

We consider three deployment trajectories, the first of which demonstrates
the value of a VIPzone approach, but has no clear path to achieving it.
The second trajectory leverages the MANRS initiative. The third trajectory,
or something similar, could derive from regulatory incentives.

\subsection{Greedy Construction of Global VIPzone} 
\label{subsec:greedyzone}

Figure~\ref{fig:solution:size-defn} shows the growth in the number of
customer ASes whose routes are protected as the VIPzone size increases.
For this analysis, we added ASes to the VIPzone to maximize the gain in
protected customers for each iteration using CAIDA's AS relationship
data (1 Dec 2022).  Customers are protected from hijacks within the zone
when they have one provider as a VIPzone member, and gain maximum benefit
when all of their providers are VIPzone members as this reduces the scope
for hijacks out of zone.  With 100 ASes, as VIPzone members,
half of the ASes in the Internet are protected from hijacks within the
zone.

\begin{figure}[t]
\centering
\includegraphics{figures/vipzone-size-defn.pdf}
\caption{With the 100 most strategically selected ASes as VIPzone members,
half of the ASes in the Internet are protected from hijacks within the zone.}
\label{fig:solution:size-defn}
\end{figure}


\subsection{Leveraging MANRS to Launch VIPzone}
\label{sec:solution:manrs}

Surprisingly, the MANRS consortium already represents a substantial
coherent topological region, which could bootstrap a VIPzone.
On 1 December 2022, MANRS had 747 ISP members (as well as 22 MANRS CDN member
organizations) participating with 906 and 25 ASNs, respectively
\cite{manrs-stats}.  (Some ISPs participate with more than one AS.) To see how
many of these are part of a coherent region,
we started with the 8 Tier-1 providers (\S\ref{sec:background:bgp})
that are MANRS members, and recursively examined their customers' ASes
to identify which were also members of MANRS.
Using CAIDA's AS2Org data set (the most recent version at time of writing, 1
Oct 2022) and AS Relationship data (1 Dec 2022)~\cite{asrank}, we found a
connected region with 452 members and 563 ASNs.  This is fewer than the number
of MANRS members, as not all members obtain transit from at least one other
MANRS member.  There are 25,330 customer ASes (owned by 22,854 organizations)
directly connected to this region.

If all the MANRS members in the currently connected region implemented the
enhanced VIPzone practices, about one-third of the ASes in the Internet,
those that are {\em directly connected} to a member of the resulting
zone today, would have their prefixes protected from hijacks in the zone.
Further, there would be incentive for the VIPzone to expand. ASes that
want their announcements protected but whose transit provider is not a
VIPzone member may be able to connect to another transit provider that
is a member, or the transit provider itself might commit to the enhanced
practices and become a member in their own right.

The Internet Society has recently launched the MANRS+ initiative
to consider how to enhance the existing MANRS framework \cite{manrs-plus}
to improve protection against routing security threats.
We consider the VIPzone proposal to be a feasible candidate enhancement. 





\subsection{U.S. Case Study}
\label{sec:usg-fcc}

Motivated by the FCC's recent Notice of Inquiry \cite{fcc-noi-2022},
we use the U.S. as a case study to explore a hypothetical
deployment scenario and its residual risks of hijacks.
We try to estimate what fraction of ASes are protected,
and the character (size, routing footprint) of those that are not protected.
For this analysis, we consider the actual Internet AS-level
topology, including provider-customer and peering relationships.
Relevant aspects of this topology, such as the AS path length
from the periphery to core (Tier 1) ISPs, varies by region and
over time. Deployment of our scheme would likely induce changes in
how AS operators configure their (transit and peering) interconnections.

Assume that the MANRS program expanded such that any U.S. network operator
(AS) with more than 100 customer ASes (aggregating across all the ASes
that belong to that organization) became part of the VIPzone.  What would
protection of the U.S. region of the Internet look like in this case?
We use data from CAIDA's AS Rank service (1 December 2022) to estimate
the number and types of ASes receiving protection from this scenario.
Note that these numbers rely on a current publicly observable state
of the Internet's AS topology, which changes as ISPs change their
interconnection patterns.  They are only an approximation to frame the
discussion.

\subsubsection{U.S. ASes with only transit interconnections}

\begin{figure}
\centering \includegraphics{figures/vipzone-7.pdf}
\caption{The shape of provider-customer connections in the U.S. region of the Internet if all organizations with more than 100 AS customers were in the VIPzone.}
\label{fig:topo}
\vskip -5mm
\end{figure}

Stipulating that all ASes with greater than 100 customer ASes
participate in VIPzone practices,
Figure~\ref{fig:topo} depicts the distribution of ASes with different
levels of protection.  An estimated 542 U.S. ASes would be in the VIPzone,
and another 14,219 customer ASes (in the teal section) would also benefit from
protection due to their direct transit connection to a provider in the
VIPzone.  These 14,219 ASes include those with the interconnection 
arrangements described in Table~\ref{tab:us}.
The first row (12,707 ASes) represents customers who only have transit providers
in the zone.  The second row (1,512 ASes) is customers that get transit
service both from provider(s) in the VIPzone and from provider(s) 
directly connected to the zone ($C_3$ in Figure~\ref{fig:topo}). 
These ASes are protected, but ASes in the VIPzone will always prefer the
prefixes of that customer that are directly announced to the VIPzone.

The remaining set of ASes do not get protection, although the 
stub ASes that are two or more hops away from the zone (1,635 + 360)
could acquire protection by choosing a transit provider in the zone,
which provides incentive for their current transit provider to join the zone.
For the 817 multi-homed ASes that are more than one hop from the zone (fifth row),
the hijack risk also remains.  In our observation period, these ASes
were small institutions, e.g., a business or school.  A policy question
is whether the risk of hijacks of these small targets is
a material concern.  The 158 ASes that received transit from a non-U.S.
provider were mostly foreign subsidiaries of U.S. firms. To understand
what protection the VIPzone could secure for these ASes would require
a hypothetical scope for the VIPzone outside the U.S., which we do not attempt.
Finally, 99 U.S. ASes had no inferred transit provider, so we did not consider 
them in this analysis.




\begin{table}
\begin{tabular}{lr}
\toprule
Connection type                                    & Number \\
\midrule
Customers with only transit provider(s)            &        \\
in VIPzone (C$_{1}$ and C$_{2}$)                    & 12,707 \\
Customers with mixed transit provider              &        \\
types (C$_{3}$)                                    &   1,512 \\
Total Protected (82.7\%):                          & {\bf 14,219} \\
\midrule
Single homed stub that are two hops from          &         \\
VIPzone (U$_{2}$)                                  &   1,635 \\
Single homed ASes that are more than two          &        \\
hops from VIPzone (U$_{3}$)                        &   360 \\
Multi-homed ASes more than one hop from           &         \\
the VIPzone (U$_{4}$, U$_{5}$, U$_{6}$)             &   817 \\
ASes with transit from non-U.S.                  &         \\
provider (U$_{8}$)                                 & 158    \\
Total Unprotected (17.3\%):                       & {\bf 2,970} \\
\midrule
Total U.S. ASes                                  & {\bf 17,189} \\
\bottomrule
\end{tabular}
\caption{Protection based on interconnection arrangements of $\approx$17K U.S. ASes 
if all U.S.~ASes with more than 100 customer ASes were required to join the VIPzone.
Note that a metric of the VIPzone's success would be that ASes changed their
interconnection arrangements to increase protection coverage offered
by the zone. Thus we intend this analysis only to illustrate the coverage
benefits of VIPzone deployment.}
\label{tab:us}
\end{table}

\subsubsection{U.S. ASes that peer outside zone}

Figure~\ref{fig:topo} depicts only transit links, i.e., between a
customer and transit provider; peering connections are so dense
that we cannot usefully visualize them.
But as mentioned in \S\ref{subsec:vipzone-peering},
peering connections have implications for protection against
hijacks. As a hypothetical case study, we examined the U.S. ISP with over
100 AS-level customers and the
largest number of peering connections: Hurricane Electric (HE).
In our data set, HE had 2079 AS-level customers, and 7677 peers
globally, of which 699 were in the U.S.  76 Of these 699 were
in the VIPzone, 536 were directly connected customers of ASes
in the VIPzone, and 30 were ASes more than one hop from the zone.
If HE were in the zone, 
when HE receives announcements from its peers not in the zone, HE should
mark them \ver~or not based on VIPzone practices \S\ref{sec:design:vipzone}.

The complication for an AS in the VIPzone with peers that are not in the
zone is that some ASes in the customer cone of one of their peers may
also have a connection to another provider that is in the VIPzone
(see \S\ref{subsubsec:transit-and-peering} and Figure~\ref{fig:transitpeering}).
HE's rich peering practices yield 2629 ASes it can reach
both through a peer not in the VIPzone (and thus using announcements that are not~\ver) and
through a peer or customer in the VIPzone, using a path that is \ver.  We assume that HE would prefer
to reach these $\approx$2K ASes over a peering connection, but for most
of them (all but 352) HE has multiple routes via peers to those ASes,
one of which is a peering path inside the VIPzone. This outcome arises
from the rich peering relationships used by HE. Only for the remaining
352 ASes would HE have to decide to forego the peering path and prefer the
\ver~option, or undertake to get accurate knowledge about the customers
of that peer, so that it could implement an exception to the preference
rule and prefer the announcement from the peer that is not \ver.

Our proposal generally assumes it is not practical for an AS to have
accurate knowledge of the customers of its customers, or in this case
its peers. However, it may be practical in specific cases.  If HE were
to prefer this route without having information about the customers of
the peer, it would put its own customers at risk of a hijack originating
in that peer.

Note that if Hurricane and Cogent agreed to peer with each other,
Hurricane would get access via the VIPzone to 220 of the 352 ASes we
consider here. Business rather than technical decisions will
determine availability of VIPzone protections to customers.  Also, 
deployment of the practices would likely lead to changes in interconnection
practices, and thus the Internet topology.


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{From zero trust to zone of trust}
\label{sec:discussion:zerotrust}

We recognize that our approach may seem at odds with the
well-founded security philosophy of {\em zero trust architectures},
and we hope to preempt related criticism by offering an explanation for this tension.
Zero trust is usually proposed in a context where each machine
or subsystem performs its own verification to protect itself, and the
incentives are directly aligned \cite{nist-zerotrust}.
The collective action aspect of
routing security is at odds with the assumptions of zero trust.

That is, if an ISP performs ROV, it typically helps the rest of the
Internet more than the ISP itself or its customers, so the deployment
incentive is low.  In our approach, allocating responsibility to specific
points in the zone (the perimeter where non-members attach to their
providers) introduces the possibility of conformance checking to ascertain
whether the trusted zone members are properly implementing the required
operational practices (\S\ref{subsec:monitoring}).

A complete zero-trust approach to routing security, where every
AS verified every BGP announcement for correctness, would
require enough authoritative data on provider-customer AS
relationships to enable this verification. One could create a new global
database, as in ASPA, or embed the data in the announcement in a
cryptographically robust manner, as in BGPsec. We discuss these two
approaches in \S\ref{sec:comparison}. However, it is inauspicious
to call for a zero-trust approach if the incentives of the actors to
implement it are not aligned, and if it is not feasible to determine if
the actors are actually performing the needed verification.

\begin{comment}

\paragraph{Multiple Trust Zones.}
We see no barrier to having multiple zones of trust. A country like China
with a domestic customer base and services local to that country could
have a zone that was local to that country.  One caveat is that for a
VIPzone to be effective, ASes that serve customers of important services
attached to that zone must also be attached to that zone. That requirement
prevents a path hijack against those services that would impact those
customers. But a small zone will provide poor protection if a service
point has global customers.  To protect itself, the service would have
to replicate its points of attachment in all the relevant zones.  To
exaggerate for effect, if each country wants its own trust zone, networks
with global customer bases would have to replicate their point of
attachments in all the trust zones where they serve customers.  Mechanically,
it is easy to isolate zones from each other--the router in one zone
receiving traffic from another zone must just delete the \ver~value from
that zone.

\end{comment}

\begin{comment}
\section{Open Issues}
\label{sec:discussion}

\kc{mjl recommends removing this section from usenix submission and putting it in another written document}
Our proposed VIPzone approach requires further analysis
to identify implementation issues and how attackers might respond to the
mechanisms.  We review several such issues.

\mypara{Trustworthy means of verification.} MANRS does not require that
members use ROAs to verify the origin announcements from their customers.
We need to understand how trustworthy other methods are, and whether
they provide a means for malicious abuse of the system.

\mypara{Other classes of MANRS participants.} It is necessary to further examine
the required practices for IXPs and CDNs interact with this proposal.

\mypara{Conformance checking.} There are details to work out
regarding conformance checking, including the challenge of checking that
members delete the \ver~value from incoming packets.

\mypara{Escalation of the threat model.}
A natural adaptation by malicious actors would be to attack the authoritative
databases that store (ROA) information about origin (and perhaps path)
validity.
This threat is well-understood---how to
secure a Internet-facing system that stores high-value information---and is
not unique to BGP.
The key question is whether loss of
access to the database should induce loss of connectivity,  or instead loss of protection from route hijacks.
Given ISP sensitivity to a loss of availability in the forwarding
service, we believe the preferable design option is to ``fail open'' in case of loss of access to authoritative databases.
This choice implies that such databases must have high availability,
including resistance to DDoS attacks and similar abuse, similar to systems such as the DNS.



\label{subsec:multiple_zones}

\mypara{Multiple trust zones}
There is no barrier to having multiple zones of trust. A country like China with a domestic customer base and services local to that country could have a zone that was local to that country.
For a VIPzone to be effective, ASes that serve customers of important
services attached to that zone must also be attached to that zone. That
prevents a path hijack against those services that would impact those
customers. But a small zone will provide poor protection if a service
point has global customers. \kc{last sentence lost me}
To protect itself, the service would have
to replicate its points of attachment in all the relevant zones.
Mechanically, it is easy to isolate zones from each other--the router
in one zone receiving traffic from another zone must just delete the
\ver~value from that zone.


\end{comment}


==> solution.tex <==
\subsection{Peering Interconnection Scenarios}
\label{subsec:vipzone-peering}
In most cases, the analysis for a peering connection is similar to transit
connections, and straightforward.

\subsubsection{Peering with IXP route servers} \label{sec:solution:ixp}

An IXP-operated route server centralizes peering routes from IXP members and
makes these routes available to other IXP members.  If the IXP is a member of
the VIPzone and has configured the route server to verify routes received from
IXP members, then the route server can mark routes as \ver, and VIPzone members
can propagate the \ver~route.  Otherwise, routes received from a route server
are unverified.

 \subsubsection{Peering of zone customers outside zone}

If two ASes not in the VIPzone but directly connected
to VIPzone providers peer with each other, they may receive announcements of
routes to each other via the VIPzone that are marked~\ver, and announcements
over the peering connection that are not \ver.  Because ASes not in the VIPzone
are not expected to use that community value to assign a preference to an
announcement, their routing policy would normally be the same as today.  (Note
ASes outside the zone may choose to use this VERIFIED value to prefer routes.)

\begin{figure} \vskip 5mm \centering
\includegraphics[width=.4\textwidth]{figures/vipzone-6.pdf}
\caption{{\em {\bf Peering across the VIPzone perimeter.} C$_{2}$ has two
transit providers, only one of which (M$_{6}$) is in the VIPzone. M$_{6}$ will
announce into the VIPzone a verified path to C$_{2}$. C$_{4}$  peers with
M$_{7}$ which is in the VIPzone. C$_{4}$ will announce to M$_{7}$ a route to
C$_{2}$. M$_{7}$ will prefer the \ver~ announcement, and will send traffic to
C$_{4}$  through its provider M$_{6}$ in the zone, not over the peering link to
C$_{4}$. }} \label{fig:transitpeering} \vskip -5mm \end{figure}


\subsubsection{Peering across the VIPzone perimeter}
\label{subsubsec:transit-and-peering}

Peering across the VIPzone perimeter has a straightforward scenario and a
complicated scenario.  Imagine that VIPzone M$_{7}$ in Figure
\ref{fig:transitpeering} peers with non-VIPzone C$_{4}$. In the straightforward
case, M$_{7}$  will apply the same VIPzone rules to peer C$_{4}$ as it does for
customers C$_{3}$ and C$_{5}$, i.e., forward or drop announcements and
mark as \ver~announcements that the peer legitimately originates. The
customers of that peer C$_{4}$ would not have their routes \ver.  Typical
routing policy is that the AS in the zone would only use these announcements
from peer  C$_{4}$ 
for itself and its customers---it would not forward them on to other
peers or providers.

The complicated peering scenario arises when a customer of that non-zone member also
obtains transit service from an AS in the VIPzone.
Figure~\ref{fig:transitpeering} shows C$_{2}$ with two transit providers, only
one of which is in the zone. The transit provider not in the zone (C$_{4}$)
also peers with an AS in the zone (M$_{7}$). In this case, M$_{7}$ will receive
a \ver~announcement to C$_{2}$ via M$_{6}$, which per the VIPzone rules it must
prefer over the route via the peering link from C$_{4}$, so M$_{7}$ will not
benefit from the peering link for traffic to C$_{2}$, even if it would
normally prefer that peering link.

In \S\ref{sec:usg-fcc}, we analyze the observable
connectivity of a major ISP, Hurricane Electric (HE), which has a liberal
peering policy, and as a result has more peers than any other ISP in the
Internet. We analyze the consequences if HE were to join the
VIPzone---in particular what residual risks might arise from the large
local region created by their peers.

\begin{comment} 
\paragraph{Potential residual risk} In general, network
operators would prefer to reach a destination using a path via a peer rather
than a path via a provider. In this specific case, AS500 might be tempted to
violate the rule that a VIPzone member must always prefer a \ver~ announcement,
and instead select the announcement from the peering link for its own use (and
that of its customers). This local policy decision would have no impact inside
the zone beyond AS 500 itself. It would be up to the operator of AS 500 to
assess the residual risk from making a local decision to prefer an announcement
that is not \ver.  This choice is an example of the balance between maximum
protection and operational flexibility to the VIPzone members.  It is an open
question whether the VIPzone should accommodate this sort of flexibility in
member routing policies and its concomitant risks. \kc{and poor AS600 might get
screwed even though he {\em only} has a provider in the zone so does not
deserve to get screwed. ;( } 
\end{comment}


